The complementary roles of non-verbal cues for Robust Pronunciation Assessment

Research on pronunciation assessment systems focuses on utilizing phonetic and phonological aspects of non-native (L2) speech, often neglecting the rich layer of information hidden within the non-verbal cues. In this study, we proposed a novel pronunciation assessment framework, IntraVerbalPA. % The framework innovatively incorporates both fine-grained frame- and abstract utterance-level non-verbal cues, alongside the conventional speech and phoneme representations. Additionally, we introduce ''Goodness of phonemic-duration'' metric to effectively model duration distribution within the framework. Our results validate the effectiveness of the proposed IntraVerbalPA framework and its individual components, yielding performance that either matches or outperforms existing research works.

==> ahmed_rs.tex <==
Computer-assisted pronunciation training (CAPT) for foreign language learning has seen a surge in global demand in recent years, driven by internet-based applications. Meanwhile, speech technology in education and CAPT has seen significant growth, thanks to advances in automatic speech recognition (ASR). CAPT benefits non-native learners with personalized, cost-effective feedback, promotes self-directed learning and improves pronunciation skills. It also offers flexibility compared to traditional instruction \cite{eskenazi2009overview,litman2018speech}.

CAPT systems have two main usages: (\textit{i}) pronunciation assessment (PA), where the system is concerned with errors in the speech segment; (\textit{ii}) pronunciation teaching, where the system is concerned with correcting and guiding the learner to fix errors in their pronunciation. PA aims to automatically score non-native speech-segment and give
meaningful feedback \cite{thomson2015effectiveness}. 






\noindent For a multilingual PA, \cite {zhang2021multilingual} proposed a unified framework for fine-grained multilingual speech evaluation, they adopted tempo-aware and phoneme-aware features in evaluation modeling, and the extracted features were inspired by music processing and vector representation learning. \cite{lin2023multi} constructed a concise unified phoneme set for multi-lingual phoneme recognition based on a wav2vec 2.0 \cite{baevski2020wav2vec}, which enables the system to share language-independent knowledge, as well as discriminating language-specific information. PA. Furthermore,  they use language-specific embeddings for different languages.

Motivated by the strong correlation between pronunciation proficiency scores and phonetic errors in non-native speech assessments of human evaluators, \cite {ryujoint} proposed a novel model architecture to multi-task both PA and mispronunciation detection and diagnosis (MDD) using wav2vec2.0, which significantly outperforms single-task learning.

\cite{shidisentangling} investigated the influence of non-native data on PA,  by examining alignment accuracy and assessment performance. They examined the impact of the proportion of non-native data in acoustic model training, their results suggested that incorporating non-native data in training can improve PA especially in a low-resource setup, where adding $10$ hours of non-native data, regardless of the type of transcriptions used, significantly improves
alignment and PA accuracy. MULTIPA \cite {chen2023multipa} is a multi-task PA that provides a precise and holistic assessment of pronunciation Skills for  closed and open response scenarios with a wide range of evaluations, encompassing assessments at both the sentence and word-level.

\noindent We build on previous research and address the gap by using paralinguistic features. Specifically, we examine phonetic representations along with non-verbal cues as auxiliary information to provide a multi-stream learning. Our contributions are:
\begin{itemize}
    \item First
    \item Second
\end{itemize}


==> intro_sac.tex <==
Computer-assisted pronunciation training (CAPT) for foreign language learning has seen a surge in global demand in recent years.
% , driven by internet-based applications. Meanwhile, speech technology in education and CAPT has seen significant growth, thanks to advances in speech technology.
% automatic speech recognition (ASR). 
CAPT benefits non-native learners with personalized, cost-effective feedback, promotes self-directed learning and improves pronunciation skills. It also offers flexibility compared to traditional instruction \cite{eskenazi2009overview,litman2018speech}.
One of the main objective of the CAPT is to automate pronunciation assessment (PA).
To achieve this goal, the automated PA model need to estimate a score that reflects the oral proficiency based on some standardized assessment criteria \cite{levy2013call, eskenazi2009overview}. 

The task of PA is inherently subjective, even scores assigned by human expert annotator often vary for the same spoken utterance. These discrepancies arises from annotator's unique experiences, their own interpretations of the scoring guidelines, and/or their focus specific aspect of pronunciation -- like fluency, prosody, word accuracy or even a combination.
Hence, designing an automated PA that emulate the annotators' (or a teacher) is very much complex and challenging. The challenges extends beyond the constraints of datasets availability, and modeling intricacies, to include the crucial task of selecting features and their representations.

Various features and modeling approach has been investigate to improve modeling performances. The studies include ....

However, majority of the studies often neglect the rich layer of information hidden within the non-verbal cues present within the nuanced layer of spoken content. For automated PA system, integrating an addition layer of non-verbal cues -- pitch, intonation, stress pattern and voice quality, can greatly enhance the system's ability to evaluate oral proficiency, bringing in the human perception factor in the equation. 

Therefore, in this study, we introduce an novel PA framework -- \textbf{IntraVerbalPA}. The framework is jointly trained to score the `fluency' and `prosodic' aspects in multi-task setup and
leverages both latent speech and phoneme embedding, while complementing them with handcrafted frame- and utterance-level non-verbal paralinguistic cues. We explored both conventional and unconventional non-verbal cues -- duration, pitch, jitter, intonation, voice and unvoiced segment features among others, for modeling PA scores. Furthermore, we introduce a novel metric to integrate the temporal information in the model.


% Our contribution are as follows: (a) explore (un)conventional non-verbal cues -- duration, pitch, jitter, intonation among others for the modeling of PA; (b) in

strengthen the `fluency' and `prosodic' representation learne by the model i

both frame- and utterance-level non-verbal cues representation to integrate the knowledge in the system.

injected these non-verbal cues in both

to enhance the model performance and its generalizability.


these over-looked handcrafted non-verbal paralinguistic cues as complementary information to provide a multi-aspect to the task.



Non-verbal cues in speech go beyond the spoken words to provide a richer, more nuanced layer of communication. These cues can include elements like intonation, pitch, speed, and pauses, as well as more subtle features like stress patterns and voice quality. While the words we say convey the explicit content of our message, non-verbal cues often reveal the emotional context, the speaker's attitude, and sometimes even their intent. In pronunciation assessment and automated speech recognition, accounting for these non-verbal cues can greatly enhance the system's ability to understand and evaluate spoken language in a way that's more aligned with human perception.


Apart from dataset limitations and modeling intricacies, selecting features to focus on is also challenging but important.


elements of pronunciation—such as fluency, prosody, or word accuracy—that they choose to emphasize.


Designing a system to emulate a teacher/rater's score, is very much challenging. The task of 


These challenges ranging from dataset limitations to feature selection and modeling intricacies.



The nature of data needed to train such model, is very much subjective. The scores given by the expert annotators often varies for a same utterance, 

on the aspect of pronunciation (prosody, fluency, word accuracy among others)  
% To design such an automated system, a model need to be trained on human annotated data. 
% Designing such dataset is, in practice, very much challenging. The annotation task is very much subjective 

 % in nature. 




The goal of automatic pronunciation assessment is for the model to estimate a score that reflects the oral proficiency. Such automated system offers 

In SLA, a rater listens to one or more spoken utterances from a student, then assigns a score. The score can be related to various possible aspects of oral proficiency, such as pronunciation ac- curacy, intonation, fluency, prosody, topic relatedness, and task completion. It is also possible to assign a holistic score that encompasses multiple of these aspects [31]. In automatic SLA, a model is trained to emulate the rater’s assigned score. This can be used to automatically assess a student’s language proficiency, and potentially be incorporated into an automatic language tutoring system. Automatic SLA may allow language education to be more accessible to a wider population, by reducing the barriers of cost and manpower.

This task is subjective in nature, meaning that different expert raters often assign different score values to the same utterance. The difference arises from the varied experiences and training backgrounds of the raters, and from a subjective interpretation of the marking rubric, which often is limited in coverage.

==> tmp.tex <==
Intelligibility and Communicative Effectiveness as Goals Rather than Correctness or Accuracy
Those who speak English as their first or native language are now in the minority, representing less than a quarter of the world’s population of English speakers, with the approximately one billion people who speak English as an L2 forming the global majority (Babbel, 2021; Statistica, 2021). The fact that much communication worldwide occurs among multilinguals who use English as their common L2 has opened discussion about appropriate goals and priorities for a pronunciation curriculum aimed at preparing language learners for communication in English as a lingua franca (ELF; Cruttenden, 2014; Jenkins, 2000, 2002; Seidlhofer, 2011) – and in general, for communication in English as an International Language (EIL) contexts (Low, 2015), including with L1 English speakers. The EIL orientation, linked to ELF and World Englishes (Kachru, 1992), has in a sense taken up the mantle of early CLT and maintained the pragmatism and the political and ethical, learner-centred, position that pronunciation should not be a focus of instruction as long as meaningful communication occurs. It has also taken a strong position regarding L2 speakers’ right to maintain a distinctive identity as a multicompetent, multilingual speaker. Accordingly, the focus in pronunciation has shifted away from a native-speaker model of correctness or accuracy to embrace L2 varieties and to assess pronunciation in terms of such general goals as intelligibility (Levis, 2018) and communicative effectiveness (Pennington and Rogerson-Revell, 2019).
